Inclusion Arena: An Open Platform for Evaluating Large Foundation Models with Real-World Apps

Large Language Models (LLMs) and Multimodal Large Language Models (MLLMs) have ushered in a new era of AI capabilities, demonstrating near-human-level performance across diverse scenarios. While numerous benchmarks (e.g., MMLU) and leaderboards (e.g., Chatbot Arena) have been proposed to help evolve the development of LLMs and MLLMs, most rely on static datasets or crowdsourced general-domain prompts, often falling short of reflecting performance in real-world applications. To bridge this critical gap, we present Inclusion Arena, a live leaderboard that ranks models based on human feedback collected directly from AI-powered applications. Our platform integrates pairwise model comparisons into natural user interactions, ensuring evaluations reflect practical usage scenarios. For robust model ranking, we employ the Bradley-Terry model augmented with two key innovations: (1) Placement Matches, a cold-start mechanism to quickly estimate initial ratings for newly integrated models, and (2) Proximity Sampling, an intelligent comparison strategy that prioritizes battles between models of similar capabilities to maximize information gain and enhance rating stability. Extensive empirical analyses and simulations demonstrate that Inclusion Arena yields reliable and stable rankings, exhibits higher data transitivity compared to general crowdsourced datasets, and significantly mitigates the risk of malicious manipulation. By fostering an open alliance between foundation models and real-world applications, Inclusion Arena aims to accelerate the development of LLMs and MLLMs truly optimized for practical, user-centric deployments. The platform is publicly accessible at https://www.tbox.cn/about/model-ranking.

==> doc/formula_derivation.tex <==
\section{Formula Derivation}

\subsection{Log-Likelihood Function}
Assume the data consists of $K$ independent matches. Each match $k$ involves models $a_k$ and $b_k$ ($a_k \ne b_k$), and the outcome $y_k \in \{0,1\}$ indicates whether model $a_k$ wins. Based on the BT-BLE model, the probability of model $a_k$ defeating model $b_k$ is defined as:
\begin{equation}
p_{k} = \sigma(\Delta r_k) = \frac{1}{1 + e^{-\alpha(r_{a_k} - r_{b_k})}}.
\label{eq:prob}
\end{equation}
where $\alpha=\frac{ln10}{400}$, and $\Delta r_k = r_{a_k} - r_{b_k}$.
Since the outcome $y_k$ follows a Bernoulli distribution, the conditional likelihood function based on \eqref{eq:prob} is calculated as:
\begin{equation}
L(\theta) = \prod_{k=1}^K \left[ \sigma(\Delta r_k)^{y_k} \left(1 - \sigma(\Delta r_k)\right)^{1-y_k} \right],
\label{eq:likelihood}
\end{equation}
where $\theta = (r_1, r_2, \dots, r_n)^T$ is the model rating vector. The log-likelihood function is:
\begin{equation}
\ell(\theta) = \sum_{k=1}^K \left[ y_k \log \sigma(\Delta r_k) + (1 - y_k) \log \left(1 - \sigma(\Delta r_k)\right) \right].
\label{eq:loglikelihood}
\end{equation}


\subsection{Fisher Information Matrix}
The Fisher Information Matrix $I(\theta)$ is defined as the negative expected value of the second derivative of the log-likelihood function:
\begin{equation}
I(\theta) = -\mathbb{E}\left[ \frac{\partial^2 \ell(\theta)}{\partial r_i \partial r_j} \middle| \theta \right].
\label{eq:fisher_def}
\end{equation}
In this case, take $\theta$ as the independent variable. Since matches are independent, the total Fisher information matrix is the sum of contributions from each match. Therefore, we first derive the Fisher information matrix $I_k$ for a single match. Consider a match between model $i$ and model $j$ ($i \ne j$), we have the outcome $y$ follows a Bernoulli distribution, where $ \mathbb{E}[y] = p_{ij} $ and $ \text{Var}(y) = p_{ij}(1 - p_{ij}) $, and the probability of model $i$ defeating model $j$ is $p_{ij}=\sigma(\Delta r_{ij})$. Thus, the log-likelihood function for this match is:
\begin{equation}
\ell_{ij} = y \log \sigma(\Delta r_{ij}) + (1 - y) \log(1 - \sigma(\Delta r_{ij})) = y \log p_{ij} + (1 - y) \log(1 - p_{ij}).
\label{eq:single_match_loglik}
\end{equation}
Taking the partial derivative with respect to the rating parameter $r_i$, we obtain the gradient:
\begin{equation}
\frac{\partial \ell_{ij}}{\partial r_i} = \left( \frac{y}{p_{ij}} - \frac{1 - y}{1 - p_{ij}} \right) p_{ij}(1 - p_{ij}) \cdot \alpha = \alpha(y - p_{ij}).
\label{eq:grad_ri}
\end{equation}
Similarly, taking the partial derivative with respect to $r_j$:
\begin{equation}
\frac{\partial \ell_{ij}}{\partial r_j} = -\alpha(y - p_{ij}).
\label{eq:grad_rj}
\end{equation}
For other models $m \ne i,j$, we have $\frac{\partial \ell_{ij}}{\partial r_m} = 0$.

Subsequently, calculate the second derivatives:
\begin{align}
\frac{\partial^2 \ell_{ij}}{\partial r_i^2} &= -\alpha^2 p_{ij}(1 - p_{ij}), \label{eq:second_deriv_ri_ri} \\
\frac{\partial^2 \ell_{ij}}{\partial r_j^2} &= -\alpha^2 p_{ij}(1 - p_{ij}), \label{eq:second_deriv_rj_rj} \\
\frac{\partial^2 \ell_{ij}}{\partial r_i \partial r_j} &= \alpha^2 p_{ij}(1 - p_{ij}). \label{eq:second_deriv_ri_rj}
\end{align}
Thus, the elements of the information matrix for a single match are:
\begin{align}
[I_{k}]_{ii} & =  -\mathbb{E}\left[ \frac{\partial^2 \ell_{ij}}{\partial r_i^2} \right] = \alpha^2 p_{ij}(1 - p_{ij}) = [I_{k}]_{jj}, \label{eq:single_match_fisher_diag} \\
[I_{k}]_{ij} &= -\mathbb{E}\left[ \frac{\partial^2 \ell_{ij}}{\partial r_i \partial r_j} \right] = -\alpha^2 p_{ij}(1 - p_{ij}). \label{eq:single_match_fisher_offdiag}
\end{align}
Meanwhile, other elements are zero. It should be noted that the term $ p_{ij}(1 - p_{ij}) $ reflects the variance of the Bernoulli outcome $ y $, which directly determines the Fisher information contributed by a single match.

Extending the result from a single match to all samples, let $c_{ij}$ denote the number of matches between models $i$ and $j$ ($i \ne j$). The elements of the total Fisher Information Matrix are:
\begin{equation}
[I(\theta)]_{ij} = \sum_{k=1}^K [I^k]_{ij} =
\begin{cases}
\sum_{m \ne i} c_{im} \alpha^2 p_{im}(1 - p_{im}), & i = j, \\ 
-c_{ij} \alpha^2 p_{ij}(1 - p_{ij}), & i \ne j \text{ and } c_{ij} > 0, \\
0, & \text{otherwise}.
\end{cases}
\label{eq:total_fisher}
\end{equation}
Here, the diagonal element $[I(\theta)]_{ii}$ represents the sum of information from all matches involving model $i$, while the off-diagonal element $[I(\theta)]_{ij}$ represents the information from matches between model $i$ and model $j$.

\subsection{MLE Estimation Precision}
The Cramer-Rao bound states that the inverse of the Fisher information is a lower bound on the variance of any unbiased estimator of $\theta$. Considering an unbiased estimator $\hat{\theta}(X)$ of $\theta$, we have:
\begin{equation}
\text{Var}(\hat{\theta}) \ge I(\theta)^{-1}.
\label{eq:cramer_rao}
\end{equation}
Note that the precision of $\theta$ is essentially limited by the Fisher information of the likelihood function.


Specifically, according to the asymptotic properties of Maximum Likelihood Estimation (MLE), assuming the Fisher information matrix is $I(\theta)$, the parameter estimator $\hat{\theta}$ follows a normal distribution for large samples:
\begin{equation}
\hat{\theta} \sim \mathcal{N}(\theta, I(\theta)^{-1}).
\label{eq:mle_asymptotic}
\end{equation}
Therefore, for the ELO rating $r_i$ of any model $i$, the variance of its unbiased estimator $\hat{r}_i$ is $[I(\theta)^{-1}]_{ii}$. From this, it can be seen that we can reduce the variance by maximizing the eigenvalues of $I(\theta)$. There are two implementation strategies:

\textbf{(1) Increase the number of matches.} The total information is proportional to $c_{ij}$, so increasing the total number of matches directly increases the scale of the information matrix.

\textbf{(2) Ensure matches are played between models of similar skill.} Observing Equation \eqref{eq:total_fisher}, it is noted that the parameter estimation precision of the ELO model directly depends on the match arrangements (i.e., the distribution of $p_{ij}$). When $p_{ij} = 0.5$ (i.e., $r_i = r_j$), $p_{ij}(1 - p_{ij})$ reaches its maximum value of $0.25$. At this point, the information contributed by a single match is maximized. By making $\Delta r_{ij}$ close to zero for each match, the information contribution of each match can be maximized, increasing $[I(\theta)]_{ij}$ and thereby reducing the variance of $\hat{r}_i$.

==> doc/midtraining.tex <==
\section{Mid-Training}

\subsection{Mid-Training Data}

\subsection{Mid-Training Evaluation}
\cite{yang2024qwen2_5}

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.0}
\setlength\tabcolsep{3.2pt}
\small
\begin{tabular}{l|ccccccc}
\toprule
& \makecell{\textbf{Gemma3-27B} \\ \textbf{Base}} & \makecell{\textbf{Qwen2.5-72B} \\ \textbf{Base}}  & \makecell{\textbf{Qwen3-30B-A3B} \\ \textbf{Base}} & \makecell{\textbf{Llama4-Scout} \\ \textbf{Base}} & \makecell{\textbf{dots.llm1} \\ \textbf{Base}} & \makecell{\textbf{Grove-Small} \\ \textbf{Base}} \\
\midrule
Architecture & Dense & Dense & MoE & MoE & MoE & MoE \\
\# Total Params & 27B & 72B & 30B & 109B & 142B & 40B \\
\# Activated Params & 27B & 72B & 3B & 17B & 14B & 3B-4B \\
\midrule
MMLU & & 86.30 & 82.70 & & & \\
MMLU Pro & & 61.40 & 56.17 & & & \\
GPQA & & 46.50 & 39.90 & & & \\
SuperGPQA & & 40.75 & 33.97 & & & \\
BBH & & 83.80 & 69.94 & & & \\
\midrule
GSM8K & & 92.95 & 89.39 & & & \\
MATH & & 59.04 & 55.66 & & & \\
\midrule
HumanEval & & 81.71 & 89.02 & & & \\
MBPP & & 76.40 & 75.00 & & & \\
MultiPL-E & & 55.70 & 62.00 & & & \\
LiveCodeBench & & 40.40 & 47.88 & & & \\
\midrule
C-Eval & & 88.40 & 88.39 & & & \\
CMMLU & & 89.50 & 86.71 & & & \\
\bottomrule
\end{tabular}
\caption{.}
\label{table:base4B_main}
\end{table}

\subsection{Architecture Settings}

\minisection{Upcycling Paradigms}

\minisection{Group Numbers}

\minisection{Activated Experts}

==> doc/posttraining.tex <==
\section{Post-Training}

\subsection{Post-Training Data}

\subsection{Post-Training Stage}

\subsection{Post-Training Evaluation}

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.0}
\setlength\tabcolsep{3.6pt}
\small
\begin{tabular}{l|ccccccc}
\toprule
& \makecell{\textbf{Gemma3} \\ \textbf{27B IT}} & \makecell{\textbf{Qwen2.5} \\ \textbf{32B Inst}} & \makecell{\textbf{Qwen3} \\ \textbf{14B}} & \makecell{\textbf{Qwen3} \\ \textbf{30B-A3B}} & \makecell{\textbf{Llama4} \\ \textbf{Scout}} & \makecell{\textbf{dots.llm1} \\ \textbf{.inst}} & \makecell{\textbf{Grove-Small} \\ \textbf{SFT}} \\
\midrule
Architecture & Dense & Dense & Dense & MoE & MoE & MoE & MoE \\
\# Total Params & 27B & 32B & 14B & 30B & 109B & 142B & 40B \\
\# Activated Params & 27B & 32B & 14B & 3B & 17B & 14B & 3B-4B \\
\midrule
MMLU & & & & & & \\
MMLU Redux & & & & & & \\
MMLU Pro & & & & & & \\
SuperGPQA & & & & & & \\
BBH & & & & & & \\
\midrule
GPQA & & & & & & \\
GSM8K & & & & & & \\
MATH & & & & & & \\
\midrule
HumanEval & & & & & & \\
MBPP & & & & & & \\
MultiPL-E & & & & & & \\
\bottomrule
\end{tabular}
\caption{.}
\label{table:chat4B_main}
\end{table}
